On Solving Quantified Bit-Vectors using Invertibility Conditions

We present a novel approach for solving quantified bit-vector formulas in Satisfiability Modulo Theories (SMT) based on computing symbolic inverses of bit-vector operators. We derive conditions that precisely characterize when bit-vector constraints are invertible for a representative set of bit-vector operators commonly supported by SMT solvers. We utilize syntax-guided synthesis techniques to aid in establishing these conditions and verify them independently by using several SMT solvers. We show that invertibility conditions can be embedded into quantifier instantiations using Hilbert choice expressions, and give experimental evidence that a counterexample-guided approach for quantifier instantiation utilizing these techniques leads to performance improvements with respect to state-of-the-art solvers for quantified bit-vector constraints.

==> algo/algo-cegqis.tex <==
%!TEX root = ../main.tex

\begin{framed}
  \setlist{nolistsep}
%  Input: formulas $\varphi$ of the form 
%         $\binde{\vec{y}\forall\vec{x}}{\psi[\vec{y}, \vec{x}]}$ 
%         with $\psi$ quantifier-free and $\fv{\psi} = \vec{y} \cup \vec{x}$
%  \\[1ex]
  $\cegqi{\selfun}(\binde{\vec{y}\forall\vec{x}}{\psi[\vec{y}, \vec{x}]})$
  \vspace{.7ex}
  \begin{itemize}[leftmargin=1em]
    \item[\ ]  $\Gamma := \emptyset$
    \item[\ ] Repeat:
    \begin{enumerate}
      \item If $\Gamma$ is $T$-unsatisfiable, then return ``unsat''.
      \item 
      \label{cegqi:s2}
      Otherwise, if $\Gamma' = \Gamma \cup \{ \lnot \psi[\vec y, \vec{x}] \}$ is
      $T$-unsatisfiable, then return ``sat''. 
      \item Otherwise, let $\I$ be a model of $T$
      and $\Gamma'$ and $\vec{t} = \selfun( \vec x, \psi, \I, \Gamma )$. 
      $\Gamma \coloneqq \Gamma \cup \{ \psi[\vec y, \vec{t}] \}$. 
    \end{enumerate}
  \end{itemize}
\end{framed}



==> algo/algo-sc.tex <==
%!TEX root = ../main.tex

\begin{framed}
  \setlist{nolistsep}
  $\selfunbv{c}( \vec x, \psi, \I, \Gamma )$\hspace{1em} where $c \in \{
  \vspace{1ex}
  \cfgmval, \cfgkeep, \cfgeqs, \cfgeqb \}$
  \begin{enumerate}[leftmargin=1em]
    \item[\ ] Let $M = \{ \ell \mid \I \models \ell, \ell \in \lits{\psi} \}$, 
    $N = \{ \project{c}( \I, \ell ) \mid \ell \in M \}$.
    \item[\ ] For $i=1,\ldots,n$ where $\vec x = ( x_1, \ldots, x_n )$:
    \begin{enumerate}
      \item[\ ] 
      Let $N_i = \bigcup_{\ell[ x_1, \ldots, x_{i-1} ] \in N} \linearize{x_i}{\I}{\ell[ t_1, \ldots, t_{i-1} ] }$.
%      \item[\ ] If $N_i$ is non-empty, let $t_i = \solvelit{ x_i, \ell }$ for some $\ell \in N_i$.
%      \item[\ ]Otherwise, let $t_i = x_i^\I$.
      \item[\ ] 
      Let
      $
      t_i =
      \begin{cases}
        \solvelit{ x_i, \choosef(N_i) } & 
        \text{if } N_i \text{ is non-empty}\\
        x_i^\I & \text{otherwise}
      \end{cases}
      $
      \item[\ ]  $t_j \coloneqq t_j \{ x_i \mapsto t_i \}$ for each $j<i$.
    \end{enumerate}
    \item[\ ] Return $( t_1, \ldots, t_n )$.
  \end{enumerate}
  \vspace{2ex}
  {%
    \renewcommand{\arraystretch}{1.2}%
    \begin{tabular}{ll@{\hskip 1.5em}ll}
      $\project{\cfgmval}( \I, s \rel t )$ &:
        return $\top$ &
      $\project{\cfgeqs}( \I, s \rel t )$ &:
        return $s \teq t + ( s - t )^\I$ \\
      $\project{\cfgkeep}( \I, s \rel t )$ &:
        return $s \rel t$ &
      $\project{\cfgeqb}( \I, s \rel t )$ &:
        return
        $
        \begin{cases}
          s \teq t &
            \text{if } s^\I = t^\I \\
          s \teq t + 1 &
            \text{if } s^\I > t^\I \\
          s \teq t - 1 &
            \text{if } s^\I < t^\I \\
        \end{cases}
        $
    \end{tabular}
  }
\end{framed}



==> algo/algo-solve.tex <==
%!TEX root = ../main.tex

%\begin{comment}
%\begin{framed}
%  \setlist{nolistsep}
%  \solvelit{x, e[x] \rel t}:
%  \vspace{1ex}
%  \begin{enumerate}[leftmargin=1em]
%    \item[\ ]
%      If $e[x] = x$
%      \begin{enumerate}[leftmargin=2em]
%        \vspace{.5ex}
%        \item[\ ] If $\rel\;\in \{\teq\}$ then return $t$
%        \item[\ ] else return
%                $\choice{y}{(\getsc{x}{x \rel t} \rightarrow y \rel t)}$.
%      \end{enumerate}
%
%      \vspace{.5ex}
%      \item[\ ]
%        Assert $e[x] = \diamond (e_1, ..., e_n)$
%        for $n > 0$
%        and $x \in \fv{e_i}$
%        and $x \not\in \fv{e_j}$ for $i \neq j$.
%      \item[\ ]
%          If $\rel\;\in \{\teq, \tneq\}$
%          and $\op \in \{ \bvnotf, \bvnegf, \bvaddf \}$
%          then
%          $t' = \getinverse{e_i}{e[x] \rel t}$
%      \item[\ ]
%          else
%          $t' = \choice{y}{(\getsc{e_i}{e[x] \rel t} \rightarrow
%              %\rightarrow e[x]\{e_i \slash y \} 
%              \diamond (e_1, ..., e_{i-1}, y, e_{i+1}, ..., e_n)
%              \rel t)}$.
%      \item[\ ] Return \solvelit{x, e_i \teq t'}.
%    \end{enumerate}
%\end{framed}
%\end{comment}

\begin{framed}
  \setlist{nolistsep}
  \solvelit{x, e[x] \rel t}:
  \vspace{1ex}
  \begin{enumerate}[leftmargin=1em]
    \item[\ ]
      If $e = x$
      \begin{enumerate}[leftmargin=2em]
        \vspace{.5ex}
        \item[] If $\rel\;\in \{\teq\}$ then return $t$
        \item[] else return
          $\choice{y}{(\imp{\getsc{x}{x \rel t}}{y \rel t})}$.
      \end{enumerate}

      \vspace{.5ex}
      \item[\ ]
        else $e = \diamond (e_1, \ldots, e_i[x], \ldots, e_n)$
        with $n > 0$
        and $x \not\in \fv{e_j}$ for all $j \neq i$.
      \begin{enumerate}[leftmargin=2em]
        \vspace{.5ex}
      \item[\ ] Let $d[x'] = \diamond (e_1, \ldots, e_{i-1}, x', e_{i+1}, \ldots, e_n)$ 
         where $x'$ is a fresh variable.
        \item[\ ]
            If $\rel\;\in \{\teq, \tneq\}$
            and $\op \in \{ \bvnotf, \bvnegf, \bvaddf \}$
        \item[\ ]
            then let $t'= \getinverse{x'}{d[x'] \teq t}$ and
            return \solvelit{x, e_i \rel t'}
        \item[\ ]
            else
            let $\ic = \getsc{x'}{d[x'] \rel t}$ and
            return
            \solvelit{x, e_i \teq \choice{y}{(\imp{\ic}{d[y] \rel t})}}.
      \end{enumerate}
    \end{enumerate}
\end{framed}


==> proofs/proof-cegqi.tex <==
We show each part of the theorem below.
Note that by the definition of $\cegqi{\selfun}$ and 
since $\selfun$ is a selection function, all inputs $\I$ and $\Gamma$ 
given to $\selfun$ in the loop of this function are legal inputs.
Also note that for the first two parts, 
we have that $\cegqi{\selfun}( \varphi )$ terminates
in a state where $\Gamma$
is a set of formulas of the form $\psi[ \vec{y}, \vec{t} ]$
where, since $\selfun$ is a selection function,
\vec{t} is a tuple of $\choicef$-valid terms and 
$\fv{\vec{t}} \subseteq \vec{y}$.

Part 1) 
By definition of $\cegqi{\selfun}$,
if $\cegqi{\selfun}( \varphi )$ returns ``unsat'',
then $\Gamma$ is $T$-unsatisfiable.
By the definition of $\cegqi{\selfun}$,
we have that $\Gamma$ is a set of formulas 
of the form $\psi[ \vec{y}, \vec{t} ]$.
For each $\psi[ \vec{y}, \vec{t} ] \in \Gamma$,
we have that \vec{t} is $\choicef$-valid since $\selfun$ 
is a selection function, and hence
$\forall \vec{x} \psi[ \vec{y}, \vec{x}] \limpl \psi[ \vec{y}, \vec{t} ]$
holds in all models of $T$.
Since $\Gamma$ is $T$-unsatisfiable, 
$\forall \vec{x} \psi[ \vec{y}, \vec{x}]$ is $T$-unsatisfi\-able,
and hence $\varphi$ is as well.

Part 2) 
By definition of $\cegqi{\selfun}$,
if $\cegqi{\selfun}( \varphi )$ returns ``sat'', the
$\Gamma$ is $T$-satisfiable and 
$\Gamma' = \Gamma \cup \{ \lnot \psi[\vec{y}, \vec{x}] \}$ is
$T$-unsatisfiable.
For each $\psi[ \vec{y}, \vec{t} ] \in \Gamma$,
we have that $\fv{\vec{t}} \subseteq \vec{y}$ and hence
$\fv{\Gamma} \subseteq \vec{y}$.
Since $\vec{x} \not\in \fv{\Gamma}$, we have that
$\Gamma \cup \{ \binde{\vec{x}}{ \neg \psi[\vec{y}, \vec{x}] } \}$
is also $T$-unsatisfiable.
Let $\I$ be an arbitrary model of $\Gamma$.
Since $\Gamma'$ is unsatisfiable,
it must be that
$\I \not\models \binde{\vec{x}}{ \neg \psi[\vec{y}, \vec{x}] }$
and hence $\I \models \binda{\vec{x}}{ \psi[\vec{y}, \vec{x}] }$.
Thus 
$\Gamma \limpl \binde{\vec{x}}{ \neg \psi[\vec{y}, \vec{x}] }$ and hence
$\binde{\vec{y}}{\Gamma} \limpl \varphi$ holds in all models of $T$.
By the same reasoning as Part 1,
we have that 
$\varphi \limpl \binde{\vec{y}}{\Gamma}$ holds in all models as well.
Thus, $\varphi$ is equivalent to $\binde{\vec{y}}{\Gamma}$.

Part 3) 
Assume $\selfun$ is monotonic and finite for $\psi[ \vec{y}, \vec{x} ]$.
Since it is finite, let $\selfun^\ast$ be a finite set such that 
$\selfun( \vec{x}, \psi, \I, \Gamma ) \in \mathcal{S}^\ast$ for all valid 
inputs $\I, \Gamma$.
Since it is monotonic, each iteration of the loop adds a new formula
from $\selfun^\ast$ to $\Gamma$. Since $\selfun^\ast$ is finite, 
the number of iterations of this loop is bounded by the size of $\selfun^\ast$.
Hence, $\cegqi{\selfun}( \varphi )$ terminates.
\qed



==> proofs/proof-ic-choice.tex <==
First we show that 
$r = \choice{y}{(\ic \limpl \ell[y])}$ is $\choicef$-valid,
where $\ic$ is an invertibility condition for $y$ in $\ell[y]$. To do so,
since $\ell[y]$ is $\choicef$-valid,
we must show $\binde{y}{\ic \limpl \ell[y]}$ holds in all models of \tbv.
Since $\ic$ is an invertibility condition for $\ell[y]$, 
we have that $y \not\in\fv{\ic}$
and hence this formula is equivalent to $\ic \limpl \binde{y}{\ell[y]}$.
Let $\I$ be any model of \tbv that satisfies $\ic$.
Since $\ic$ is an invertibility condition for $\ell[y]$,
by Definition ~\ref{def:ic}, $\I$ satisfies $\binde{y}{\ell[y]}$ as well.
Thus, $\binde{y}{\ic \limpl \ell[y]}$ holds in all models of \tbv and hence $r$
is $\choicef$-valid.

To show 
$\ell[r] \lequiv \binde{x}{\ell[x]}$ where 
$r$ is $\choice{y}{(\ic \limpl \ell[y])}$,
first consider direction
$\binde{x}{\ell[x]} \limpl
\ell[r]$.
Let $\I$ be any model of \tbv that satisfies $\binde{x}{\ell[x]}$.
By definition of $\choicef$,
$\I$ also satisfies $\ell[\choice{y}{\ell[y]}]$.
Since $\ic$ is an invertibility condition for $\ell[x]$,
from Def.~\ref{def:ic}
we have that
$\ic \lequiv \binde{y}{\ell[y]}$ holds in all models of \tbv,
and thus $\I$ also satisfies $\ic$.
Hence, since $\I$ satisfies $\ell[\choice{y}{\ell[y]}]$, it also 
satifies $\ell[\choice{y}{(\ic \limpl \ell[y])}]$,
which is $\ell[r]$.
Thus,
$\binde{x}{\ell[x]} \limpl
\ell[r]$
is \tbv-valid.
%
The other direction
$\ell[r] \limpl
\binde{x}{\ell[x]}$
trivially holds in all models of~\tbv.
\qed



==> proofs/proof-sel-bv-prop.tex <==
Let \vec{x = ( x_1, \ldots, x_n )} be a tuple of variables
and let $\varphi$ be a quantifier-free $T_{BV}$-formula.
We show each part for the case where $n=1$; the arguments 
below can be lifted to $n>1$ in a straightforward way.
Let $\Gamma$ be a set of formulas such that $x_1 \not \in \fv{\Gamma}$,
let $\I$ be a model of $T_{BV}$ such that 
$\I \models \Gamma \cup \{ \neg \varphi \}$,
and let $t_1$ be $\selfunbv{c}( (x_1), \I, \Gamma )$.

Part 1)
To show that $\selfunbv{c}$ is a selection function,
we must show that $t_1$ is $\choicef$-valid and 
$\fv{t_1} \subseteq \fv{\varphi} \setminus \{ x_1 \}$.
Notice that for all configurations,
the value $( t_1 )$ returned by $\selfunbv{c}$ is either 
of the form $x_1^\I$ or $\solvelitf( x_1, \ell )$ 
for some $\ell \in \lits{\Gamma}$.
In the former case, we have that $t_1$ is clearly $\choicef$-valid 
and $\fv{t_1} = \emptyset$.
In the latter case, as a consequence of Theorem~\ref{thm:solve},
we have that $t_1$ is $\choicef$-valid and $\fv{t_1} \subseteq \fv{\ell}$.
We have that $\ell \in \lits{\varphi}$
and thus $\fv{\ell} \subseteq \fv{\varphi}$.
Thus, in either case, 
we have $\fv{t_1} \subseteq \fv{\varphi} \setminus \{ x_1 \}$.
Hence, $\selfunbv{c}$ is a selection function for 
$c=\cfgmval$, $\cfgkeep$, $\cfgeqs$, $\cfgeqb$.
To show these selection functions are finite for $\varphi$,
note that the number of terms of form $x_1^\I$ is finite.
Also note that the number of literals in $\lits{\varphi}$ is finite.
For each $c$ and $\ell \in \lits{\varphi}$, 
set of literals of the form $\project{c}( \I, \ell )$, 
call this set $N$, is finite.
For each literal $\ell' \in N$, the set of literals
returned by $\linearizef( x_i, \I, \ell' )$, call this set $N'$,
is also finite.
Since it is either the case that 
$t_1 = \solvelitf( x_1, \ell'' )$ for some $\ell'' \in N'$
or $t_1 = x_1^\I$, the number of possible return values
of $\selfunbv{c}$ is finite for $( x_1 )$ and $\varphi$
for $c=\cfgmval$, $\cfgkeep$, $\cfgeqs$, $\cfgeqb$.

Part 2)
Since $x_1 \not\in \fv{\ell}$ for any literal returned by
$\project{\cfgmval}( \I, \ell )$, it must be the case that $t_1 = x_1^\I$.
Assume that $\project{\cfgmval}$ was not monotonic
for $( x_1 )$ and $\varphi = \neg \psi[ x_1 ]$.
Since $\project{\cfgmval}$ is a selection function by Part 1
and $\I, \Gamma$ is a legal input to $\project{\cfgmval}$,
then without loss of generality we may assume that
$\psi[ t_1 ] \in \Gamma$.
However, 
$\neg \psi[ x_1 ] \in \Gamma$, $\I \models \Gamma$ and since
$t_1^\I = x_1^\I$, 
it must instead be the case that $\varphi[ t_1 ] \not\in \Gamma$.
Hence, $\project{\cfgmval}$ is monotonic for $\varphi$.

Part 3)
Assume $\varphi$ is the unit linear invertible
formula $\ell$.
%where by definition $\ell$ is linear with respect to $x_1$.
By definition of $\project{\cfgkeep}$, $\linearizef$,
and since by definition $\ell$ is linear with respect to $x_1$
and $\I \models \neg \ell$,
we have that $t_1$ must
be the term returned by $\solvelitf( x_1, \neg \ell )$.
Hence, $\selfunbv{\cfgkeep}$ has only one possible return value
and hence is $1$-finite.

Part 4)
Assume $\varphi$ is a unit linear invertible
formula $\ell[ x_1 ]$.
The return value of $\selfunbv{\cfgkeep}$ is the tuple $( t_1 )$,
where by the reasoning in Part 3, we have that $t_1$ is the term returned by
$\solvelitf( x_1, \neg \ell[ x_1 ] )$.
Thus by Theorem~\ref{thm:solve},
we have that 
$\neg \ell[t_1] \lequiv \binde{z}{\neg \ell[z]}$ holds in all models of \tbv.
Now, assume that $\project{\cfgkeep}$ was not monotonic 
for $( x_1 )$ and $\ell[ x_1 ]$.
Since $\project{\cfgkeep}$ is a selection function by Part 1
and $\I, \Gamma$ is a legal input to $\project{\cfgkeep}$,
then without loss of generality we may assume that $\ell[ t_1 ] \in \Gamma$.
Since $\I \models \Gamma$,
and since 
$\neg \ell[t_1] \Leftarrow \binde{z}{\neg \ell[z]}$ 
holds in all models of \tbv,
we have that $\I$ must satisfy $\neg \binde{z}{\neg \ell[z]}$,
which is $\binda{z}{\ell[z]}$.
However, we also have that by assumption $\neg \ell[ x_1 ] \in \Gamma$.
Hence, 
it must instead be the case that $\varphi[ t_1 ] \not\in \Gamma$
and thus $\project{\cfgkeep}$ is monotonic for $\varphi$.
\qed



==> proofs/proof-solve.tex <==
We assume without loss of generality 
that $\ell[x]$ is of the form $e[x] \rel t$.
Since $\ell[x]$ is linear with respect to $x$, we have that 
$x \not\in \fv{t}$.
We show all statements of the Theorem 
by structural induction on the term $e[x]$.

Consider the case when $e[x]$ is $x$.
If $\rel$ is $\teq$, then $r$ is $t$.
We have that $r$ is $\choicef$-valid,
$x \not\in \fv{r}$ since $x \not\in \fv{t}$ and 
$t \teq t \lequiv \binde{x}{ x \teq t}$
holds in all models of \tbv.
Otherwise, when $\rel$ is not $\teq$, we have that $r$ is 
$\choice{y}{(\psi \limpl y \rel t)}$ where
$\psi$ is $\getsc{x'}{x' \rel t}$.
By definition of $\getscf$, we have that $\fv{\psi} \subseteq \fv{t}$,
and hence $\fv{r}$ is a subset of $\fv{t}$, 
which is equal to $\fv{ \ell[x] } \setminus \{ x \}$.
Furthermore, since $\psi$ is an invertibility condition for $x'$ in $x' \rel t$,
by Lemma~\ref{lem:ic-choice},
$r$ is $\choicef$-valid and
$r \rel t \lequiv \binde{x}{x \rel t}$.
  
Otherwise, $e[x]$ must be of the form $\diamond (e_1, ..., e_i[x], ..., e_n)$ 
for $n > 0$, where
$x \not\in \fv{e_j}$ for each $i \neq j$.
Let $d[x']$ be 
$\diamond (e_1, ..., e_{i-1}, x', e_{i+1}, ... e_n)$ where
notice that $x \not \in \fv{d[x']}$.
We have that $r$ is $\solvelit{x, e_i[x] \rel_i t_i }$ 
for some relation $\rel_i$ 
and term $t_i$, where $t_i$ is either
$\getinverse{x'}{d[x'] \teq t}$ or 
$\choice{y}{(\getsc{x'}{d[x'] \rel t} \limpl d[y] \rel t)}$.
In both cases, by definition of $\getinversef$ and $\getscf$,
we have that $t_i$ is 
$\choicef$-valid due to Lemma~\ref{lem:ic-choice} and
since $\ell[x]$ is $\choicef$-valid.
Also in both cases, we have that
$\fv{t_i} \subseteq \fv{t} \cup \fv{d[x']} \setminus \{ x' \}
\subseteq \fv{\ell[x]} \setminus \{ x \}$.
Since $e[x] \rel t$ is $\choicef$-valid and linear with 
respect to $x$ and $x \not\in \fv{t_i}$, the literal $e_i[x] \rel_i t_i$
is $\choicef$-valid and linear with respect to $x$ as well.
Thus, by the induction hypothesis, we have that 
$r$ is $\choicef$-valid,
$\fv{r} \subseteq \fv{e_i[x] \rel_i t_i} \setminus \{ x \}$ and the formula
$e_i[r] \rel_i t_i \lequiv \binde{x}{e_i[x] \rel_i t_i}$
holds in all models of \tbv.

Since $\fv{r} \subseteq \fv{e_i[x] \rel_i t_i} \setminus \{ x \}$
and since $\fv{e_i[x]} \subseteq \fv{\ell[x]}$ 
and $\fv{t_i} \subseteq \fv{\ell[x]}$, we have that
$\fv{r} \subseteq \fv{\ell[x]} \setminus \{ x \}$.  

It remains to show 
$e[r] \rel t \lequiv \binde{x}{e[x] \rel t}$.
In the case that $\rel\;\in \{\teq, \tneq\}$
and $\op \in \{ \bvnotf, \bvnegf, \bvaddf \}$, 
we have that 
$\rel_i$ is $\rel$ and 
$t_i$ is $\getinverse{x'}{d[x'] \teq t}$.
By definition of $\getinversef$ and 
since $\rel\;\in \{\teq, \tneq\}$, 
we have that 
$e_i[x] \rel t_i$ and $d[e_i[x]] \rel t$ are equivalent.
Since $d[e_i[x]] = e[x]$, the latter literal is $e[x] \rel t$.
Thus,
since $e_i[r] \rel t_i \lequiv \binde{x}{e_i[x] \rel t_i}$,
we have that 
$e[r] \rel t \lequiv \binde{x}{e[x] \rel t}$.
Otherwise, we have that $\rel_i$ is $\teq$ and $t_i$ is
$\choice{y}{(\getsc{x'}{d[x'] \rel t} \limpl d[y] \rel t)}$.
Since $\psi$ is an invertibility condition for $x'$ in $d[x'] \rel t$,
by Lemma~\ref{lem:ic-choice}, we have that
$d[t_i] \rel t \lequiv \binde{x_i}{d[x_i] \rel t}$
holds in all models of \tbv.
Clearly $e[r] \rel t \limpl \binde{x}{e[x] \rel t}$
holds in all models of \tbv.
Now, consider any model $\I$ of \tbv that satisfies
$\binde{x}{e[x] \rel t}$. 
Since $e[x] = d[e_i[x]]$, we have that $\I$ satisfies 
$\binde{x_i}{d[x_i] \rel t}$ as well.
Thus, since $d[t_i] \rel t \lequiv \binde{x_i}{d[x_i] \rel t}$
holds in all models of \tbv, we have that
$\I$ satisfies $d[t_i] \rel t$.
Notice that $\I$ satisfies $\binde{x}{d[e_i[x]] \rel t}$ by assumption
and $\I$ satisfies $d[t_i] \rel t$.
Thus, since $t_i$ is $\choice{y}{(\psi \limpl d[y] \rel t)}$,  
we have that $\binde{x_i}{e_i[x_i] \teq t_i}$.
Since by the induction hypothesis
$e_i[r] \teq t_i \lequiv \binde{x}{e_i[x] \teq t_i}$
holds in all models of \tbv, we have that
$\I$ satisfies $e_i[r] \teq t_i$.
Thus, since $\I$ satisfies $d[t_i] \rel t$, we have that
$\I$ also satisfies $d[e_i[r]] \rel t$, which is $e[r] \rel t$.
Thus, $e[r] \rel t \Leftarrow \binde{x}{e[x] \rel t}$
holds in all models of \tbv.
\qed


